Is a 3D-Tokenized LLM the Key to Reliable Autonomous Driving?

Rapid advancements in Autonomous Driving (AD) tasks turned a significant shift toward end-to-end fashion, particularly in the utilization of vision-language models (VLMs) that integrate robust logical reasoning and cognitive abilities to enable comprehensive end-to-end planning. However, these VLM-based approaches tend to integrate 2D vision tokenizers and a large language model (LLM) for ego-car planning, which lack 3D geometric priors as a cornerstone of reliable planning. Naturally, this observation raises a critical concern: Can a 2D-tokenized LLM accurately perceive the 3D environment? Our evaluation of current VLM-based methods across 3D object detection, vectorized map construction, and environmental caption suggests that the answer is, unfortunately, NO. In other words, 2D-tokenized LLM fails to provide reliable autonomous driving. In response, we introduce DETR-style 3D perceptrons as 3D tokenizers, which connect LLM with a one-layer linear projector. This simple yet elegant strategy, termed Atlas, harnesses the inherent priors of the 3D physical world, enabling it to simultaneously process high-resolution multi-view images and employ spatiotemporal modeling. Despite its simplicity, Atlas demonstrates superior performance in both 3D detection and ego planning tasks on nuScenes dataset, proving that 3D-tokenized LLM is the key to reliable autonomous driving. The code and datasets will be released.

==> sections/ablation.tex <==
\section{Experiments}
We assess the performance of our autonomous driving model, Atlas, using a specialized fine-tuning dataset derived from NuScenes.

\subsection{Dataset and Metrics}
\textbf{Dataset.} Unlike typical approaches in motion planning tasks, which are not suitable for VLMs, we tailor the nuScenes dataset for both the training and testing phases in our experiments. The dataset is comprehensive, encompassing 1,000 diverse urban scenes with around 40,000 key-frames, primarily including multi-view camera images, and dynamic information such as velocity and acceleration of each frames. we have reformatted the data into multiple QA pairs. This format involves crafting questions that guide the LLMs to perform motion planning by observing and analyzing queries, which are derived from advanced 3D tokenizers. The answers, on the other hand, are constructed to demonstrate a 'chain-of-thought' reasoning process. This process starts with predictions of velocity and acceleration and progresses methodically toward detailed motion planning.

\textbf{Metrics.} We adhered to standard practices by utilizing the implementation provided by ST-P3 to assess our motion planning outputs over time horizons of 1s, 2s, and 3s. We assessed the performance with two widely accepted metrics: the L2 error calculated by comparing the predicted trajectories of the ego vehicle with the ground-truth trajectories at corresponding waypoints, and the collision rate calculated by checking for any intersections between the ego vehicle and other entities within the scene, such as other vehicles and pedestrians.

\subsection{Implementation Details}
The whole model trains with 8 Tesla A100 GPUs, with training times of approximately 100 hours.

\textbf{3D tokenizers as perceptrons pre-training.} We begin by pre-training two distinct 3D tokenizers: StreamPETR and TopoMLP, tailored for specific perception tasks. 
StreamPETR is designed for multi-view 3D object detection. We adhere to the prescribed settings, utilizing a ViT-L backbone, and process images at a high resolution of 800x1600. Moreover, we follow the official training schedule established for the nuScenes dataset.
TopoMLP, on the other hand, focuses on constructing HD maps from multiple views. To maintain methodological consistency with StreamPETR, we employ the same ViT-L backbone and resolution. The training strategy for TopoMLP also mirrors the official, it specifically utilizes `subset\_b' of the Openlane-V2 dataset, which is a subset of the nuScenes.

%We first pre-train our 3D tokenizers aka StreamPETR and TopoMLP in respective perception tasks. For StreamPETR, a multi-views 3D object detection model, we follow the official setting composed of ViT-L backbone, higher image resolution of $800x1600$, and the same training schedule, which is based on standard nuScenes datasets. For TopoMLP, a multi-views HD map construction model, we conduct the same ViT-L backbone for inner alignment with the detection model and follow the same training strategy with official produce, based on Openlane-V2 'subset_b' developed from nuScenes.


\textbf{Planning.} For motion planning,  our system, which we refer to as Atlas, integrates the 3D tokenizers described earlier with an LLM, specifically the Vicuna-1.5. This LLM has been pre-trained on a diverse open-world data corpus, providing a robust foundation for understanding and processing spatial-temporal. Atlas follows most of the basic settings in Merlin, with a batch size of 1, a learning rate of 2e-5, and the AdamW optimizer with a weight decay of 1e-4. We implement a linear warm-up phase consisting of the first 3\% steps in total. Following the warm-up, we transition to a cosine learning rate strategy. The maximum length of prompt tokens is 4096, and the number of tokens for each 3D tokenizer is 256 per frame, the memory queue stores queries of 3 additional frames. A notable aspect of our setup is we initialize the positional embeddings of the queries to zero.

\input{table/table_planning_main}

\subsection{Main Results}

In this section, we evaluate the performance of our proposed method, Atlas, by comparing it against existing state-of-the-art (SoTA) BEV-based planners, as detailed in Table \ref{tbl:planning}. Our experimental results reveal that Atlas achieves substantial improvements over the SoTA methods, reducing the average L2 metric by {\color{red}{40.0\%}} and the average Collision metric by {\color{red}{60.6\%}}. These significant enhancements corroborate the effectiveness of the 3D-tokenized LLMs, which we consider as the key to reliable autonomous driving.

Further, to ascertain whether the performance improvements are solely attributable to the inclusion of ego state information—a frequent topic of discussion within the community—we conducted additional experiments by removing the ego state data from both the training and testing phases.
In this experimental setting, compared to the prevailing VLM-based methods, our Atlas demonstrates superior performance and robustly validates the effectiveness of 3D tokenizers.
Despite this, Atlas continued to outperform other BEV-based methods in terms of collision rates. However, the performance on the L2 metric was comparable to other methods. We hypothesize that this outcome may stem from the inherent capabilities of the LLM to predict multiple potential motion trajectories and make rational decisions, which, while confronted with novel scenarios, deviate from the ground truth.

%In this section, we evaluate the performance of our proposed method, Atlas, against existing state-of-the-art (SoTA) BEV-based planners as summarized in Table \ref{tbl:planning}. Our experimental results demonstrate that Atlas achieves substantial improvements over the SoTA methods, reducing the average L2 metric by {\color{red}{40.0\%}} and the average Collision metric by {\color{red}{60.6\%}}. These significant enhancements further substantiate the effectiveness of the 3D-tokenized LLMs, which we consider crucial for reliable autonomous driving.

%To investigate whether the observed performance improvements are solely attributable to the ego state information provided during training and testing—an idea widely discussed in the community—we conducted additional experiments. We removed the ego state data from both the training and testing phases and found that Atlas still outperformed BEV-based methods in terms of collision rates. However, we noted a noticeable comparable performance in the L2 metric when compared to others. We speculate that this potential is caused by the capabilities of LLM, which could predict multiple potential motion trajectories, and make multiple rational decisions but deviate from the ground truth.

% We compare the proposed Atlas with previous state-of-the-art BEV-based planners in Tab. \ref{tbl:planning}. The experiments strongly prove that our Atlas make significant progress in both average L2 metric {\color{red}{(-40.0\%)}} and average Collision metric {\color{red}{(-60.6\%)}} compared to respective SoTA. The advances we make further evidence the validity of 3D tokenizers LLM, as we say the key to reliable autonomous driving. 
% We go one step further and evaluate whether performance improvement only comes from the ego status we provided, as has been widely discussed in the community. Even eliminating the ego states we used in the training and testing phase, our Atlas maintains the leading position in collision rate compared to BEV-based methods. However, a decrease compared to BEV-Planner in L2 is prominent, we speculate that this is due to potential speed and acceleration leakage caused by its concatenate operation to the BEV feature, but since it is not open source, we did not verify our hypothesis.


\subsection{Analysis and Ablation}
To avoid unnecessary misunderstandings, our ablation did not introduce any ego states.

\input{table/table_accumulate}

\textbf{Summary of Cumulative Effect.} We conduct comprehensive ablation studies to analyze our proposed approach,
considering several key aspects: evaluating the impact of the 3D tokenizers, examining the contribution of the memory queue, validating the
position embeddings, exploring the consistency performance in 3D detection and planning, and assessing the effectiveness of chain-of-thought. Additionally, we systematically
evaluate the cumulative effects of integrating these various
components and the results are summarized in Table \ref{tbl:accumulate}.

Our experiments demonstrate that each component we developed enhances performance in both 3D detection and planning tasks. Furthermore, we observed a synergistic effect where improvements in one task appear to amplify accuracy in the other, strongly proving that the capacity to perceive the environment remains a cornerstone of reliable planning.

\input{table/table_tokenizer}

\textbf{3D tokenizers.} In our experiments, we first investigate the effectiveness of various 3D tokenizers for motion planning, which are the central enhancements introduced in our study. The results are summarized in Table \ref{tbl:tokenizer}. The tokenizers we evaluate include BevFormer (BF), PETR (PT), StreamPETR (SP), and TopoMLP (TM). Our incorporation of progressively advanced 3D perceptrons into LLM demonstrates a notable improvement in planning performance, underscoring the significance of 3D perception in achieving robust autonomous driving. Furthermore, we integrate TopoMLP to provide supplementary lane line information. This addition results in a modest enhancement in performance, suggesting the potential benefits of incorporating contextual roadway features into the motion planning process.

\input{table/table_resolution}

\textbf{Resolution.} Our approach integrates 3D tokenizers with adjustable image resolution capabilities. This contrasts with conventional VLM-based methods that generally employ pre-training with ViT-CLIP, which restricts image resolutions and mandates the use of square-shaped images. Such constraints do not align well with real-world applications in autonomous driving.
By utilizing our 3D tokenizers, we are able to introduce resolutions that are more appropriate for the specific requirements of autonomous driving scenarios. In our experiments, as Table \ref{tbl:resolution} presents, we observed that increasing the image resolution led to a noticeable improvement in performance. This evidence clearly indicates that our method holds significant advantages over traditional VLM techniques, particularly in terms of flexibility and efficacy in handling diverse image resolutions.

\input{table/table_position}

\textbf{Position embeddings.} A key discovery in our study is the substantial impact of position embeddings when using 3D-tokenized LLM. As illustrated in Table \ref{tbl:position}, applying any of the standard position embedding techniques to visual cues does not significantly alter the performance.
We attribute this phenomenon to the uniqueness of our tokenizers, which incorporate a Deformable Attention mechanism. This design separates the spatial (location) and feature (content) information in the attention process.
To leverage this architecture, we use the offset mappings within the Deformable Attention as the form of position embedding. This approach directly connects the spatial reasoning in the model to its attention mechanism, enhancing the model's ability to interpret complex spatial arrangements. Remarkably, this method led to notable improvements in accuracy.

\input{table/table_cot}

\textbf{Chain of thought.} In the realm of autonomous driving, recent scholarly work has converged on a key insight: the state of the ego vehicle is a pivotal factor in shaping open-loop planning strategies. With this understanding as our foundation, we present a systematic framework for motion planning that is predicated on a granular examination of the ego states. To this end, we delineate the ego states into four distinct yet interrelated dimensions: velocity (V), acceleration (A), yaw angle (Y), and the historical trajectory (T).
To evaluate the influence of each dimension, we conducted motion planning based on the predicated of these parameters. The experimental findings, as outlined in Table \ref{tbl:cot}, where 'P' denotes 'Planning'. Notably, our results diverge from prevailing research, indicating that the yaw angle and historical trajectory do not enhance the efficacy of the planning process. This counterintuitive outcome is likely a consequence of the inherent difficulties in the precise forecasting of these variables~\cite{wei2023autoregressive, Bai_2024_CVPR}.
Moreover, we discovered an intriguing aspect of our model's robustness: the sequence in which these parameters are predicted does not impact the model's performance. This suggests that altering the order of prediction—reversed—does not result in a significant increase in computational time.

\input{table/table_pretrain}

\textbf{LLM pre-training.} To assess the robustness of our model, we performed several experiments using LLMs that underwent different pre-training processes. The results, presented in the accompanying Table \ref{tbl:pretrain}, indicate that pre-training methods incorporating text-image alignment significantly enhance performance in planning. We hypothesize that the superior performance of these models stems from their multimodal training. This training approach allows the models to interpret images with greater accuracy, regardless of whether the image features are aligned with 3D tokenizers or not.
Furthermore, our experiments showed that the accuracy levels among models pre-trained with text-image alignment were notably similar. This consistency can likely be attributed to the fundamental differences between 3D and 2D image features. 

\subsection{Qualitative}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/visuali.pdf}
    \vspace{-16pt}
    \caption{\textbf{Qualitative of Atlas with diverse planning.}}
    \label{fig:caption}
    % \vspace{-.5em}
\end{figure}

We also conducted a qualitative analysis by visualizing the trajectory predictions made by Atlas. The results demonstrate that Atlas is capable of generating multiple feasible plans for autonomous driving that are not only practical but also adhere to safety standards. Specifically, Atlas successfully devises various potential routes tailored to distinct driving scenarios, including following other vehicles, lane changing, and overtaking. Importantly, Atlas effectively identifies and avoids pedestrians and cars, showcasing its robust capability in ensuring road safety.

\label{sec:ablation}






==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\section{Appendix / supplemental material}
\newpage
\appendix
\input{Styles/neurips_2024_supp}

% Optionally include supplemental material (complete proofs, additional experiments and plots) in appendix.
% All such materials \textbf{SHOULD be included in the main submission.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The author's claims made in the abstract and introduction accurately reflect the paper's contributions and scope in the section Introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The authors discuss possible limitations of their approach in the section Conclusion and Limitations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper describes the architecture clearly and fully for reproducing the results or a way to reproduce the model in section 3. The code and dataset will be provided publicly soon.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code and dataset will be provided publicly soon.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The full details and experimental setting are in the section Implementation and supplemental material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Error bars are not included since running experiments multiple times is too computationally expensive.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper indicates the type of computing worker GPU in the section Implementation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We read the ethics review guidelines carefully and ensured that our paper conforms to them. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  The paper discusses both potential positive societal impacts and negative societal in the section Broader Impacts within supplemental material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The authors cite the original paper that produced the code package or dataset stating which version of the asset is used in reference.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> table/table_accumulate.tex <==
\setlength\intextsep{6pt}
\begin{wraptable}{h}{0.45\linewidth}
\footnotesize
\centering
\vspace{-2mm}
\vspace{1mm}
	   \setlength{\abovecaptionskip}{0cm}
	   \setlength{\belowcaptionskip}{0.1cm}
         \centering
  	\resizebox{0.45\textwidth}{!}{
		\setlength\tabcolsep{4pt}
		\renewcommand\arraystretch{1}
		\begin{tabular}{l|cc|cc}
    \toprule
    \multicolumn{1}{l|}{\multirow{2}*{}} & \multicolumn{2}{c|}{3D Detection} & \multicolumn{2}{c}{Planning} \\
    & \textbf{F1$_{1.0}$} & \textbf{F1$_{2.0}$} & \textbf{Avg. L2} & \textbf{Avg. Col.}\\
    \midrule
    Vicuna & 5.4 & 10.1 & 2.19 & 2.75  \\
    $+$ CoT & 5.4 & 10.1 & 1.80 & 1.20 \\
    $+$ 3D & 30.7 & 41.2 & 1.22 & 0.62 \\
    $+$ PE & 34.6 & 46.5 & 1.10 & 0.44 \\
    $+$ MQ & 39.8 & 49.7 & 1.00 & 0.38 \\ 
    \bottomrule
    \end{tabular}}
% \vspace{1mm}
\label{tbl:accumulate}
\caption{Summary of cumulative effects. CoT, 3D, PE, and MQ respectively represent Chain-of-Thought, 3D tokenizers, Position Embedding, and Memory Queue.
}  
\end{wraptable}

==> table/table_position.tex <==
\setlength\intextsep{6pt}
\begin{wraptable}{h}{0.25\linewidth}
\footnotesize
\centering
\vspace{-2mm}
\vspace{1mm}
	   \setlength{\abovecaptionskip}{0cm}
	   \setlength{\belowcaptionskip}{0.1cm}
         \centering
  	\resizebox{0.25\textwidth}{!}{
		\setlength\tabcolsep{4pt}
		\renewcommand\arraystretch{1}
		\begin{tabular}{c|cc}
    \toprule
    pos. enc. & \textbf{Avg. L2} & \textbf{Avg. Col.}\\
    \midrule
    none & 1.18 & 0.57 \\
    sin-cos & 1.21 & 0.57 \\
    learned & 1.19 & 0.56 \\
    deformable & 1.00 & 0.38 \\
    \bottomrule
    \end{tabular}}
% \vspace{1mm}
\label{tbl:position}
\caption{Effective of position embeddings.
}  
\end{wraptable}

==> table/table_pretrain.tex <==
\setlength\intextsep{6pt}
\begin{wraptable}{h}{0.25\linewidth}
\footnotesize
\centering
\vspace{-2mm}
\vspace{1mm}
	   \setlength{\abovecaptionskip}{0cm}
	   \setlength{\belowcaptionskip}{0.1cm}
         \centering
  	\resizebox{0.25\textwidth}{!}{
		\setlength\tabcolsep{4pt}
		\renewcommand\arraystretch{1}
		\begin{tabular}{c|cc}
    \toprule
    Pre-training & \textbf{Avg. L2} & \textbf{Avg. Col.}\\
    \midrule
    LLama & 1.14 & 0.47 \\
    LLava & 1.03  & 0.39  \\
    Vicuna & 1.00 & 0.38  \\
    Merlin & 0.99  & 0.42  \\
    \bottomrule
    \end{tabular}}
% \vspace{1mm}
\label{tbl:pretrain}
\caption{Effective of the variable pre-trianed LLM.
}  
\end{wraptable}

==> table/table_resolution.tex <==
\setlength\intextsep{6pt}
\begin{wraptable}{h}{0.35\linewidth}
\footnotesize
\centering
\vspace{-2mm}
\vspace{1mm}
	   \setlength{\abovecaptionskip}{0cm}
	   \setlength{\belowcaptionskip}{0.1cm}
         \centering
  	\resizebox{0.35\textwidth}{!}{
		\setlength\tabcolsep{4pt}
		\renewcommand\arraystretch{1}
		\begin{tabular}{c|cc}
    \toprule
    Resolution & \textbf{Avg. L2} & \textbf{Avg. Col.}\\
    \midrule
    336$\times$336 & 1.66 & 0.94 \\
    320$\times$800 & 1.41 & 0.58 \\
    800$\times$1600 & 1.00 & 0.38 \\
    \bottomrule
    \end{tabular}}
% \vspace{1mm}
\label{tbl:resolution}
\caption{Effective of resolution.
}  
\end{wraptable}

==> table/table_tokenizer.tex <==
\setlength\intextsep{6pt}
\begin{wraptable}{h}{0.35\linewidth}
\footnotesize
\centering
\vspace{-2mm}
\vspace{1mm}
	   \setlength{\abovecaptionskip}{0cm}
	   \setlength{\belowcaptionskip}{0.1cm}
         \centering
  	\resizebox{0.35\textwidth}{!}{
		\setlength\tabcolsep{4pt}
		\renewcommand\arraystretch{1}
		\begin{tabular}{cccc|cc}
    \toprule
    BF & PT & SP & TM & \textbf{Avg. L2} & \textbf{Avg. Col.}\\
    \midrule
    \ding{52} & - & - & \ding{56} & &\\
    - & \ding{52} & - & \ding{56} & 1.51 & 1.05\\
    - & - & \ding{52} & \ding{56} & 1.06 & 0.41\\
    - & - & \ding{52} & \ding{52} & 1.00 & 0.38\\
    \bottomrule
    \end{tabular}}
% \vspace{1mm}
\label{tbl:tokenizer}
\caption{Effective of different 3D tokenizers.
}  
\end{wraptable}
